Fusing Models with Complementary Expertise

Training AI models that generalize across tasks and domains has long been among the open problems driving AI research. The emergence of Foundation Models made it easier to obtain expert models for a given task, but the heterogeneity of data that may be encountered at test time often means that any single expert is insufficient. We consider the Fusion of Experts (FoE) problem of fusing outputs of expert models with complementary knowledge of the data distribution and formulate it as an instance of supervised learning. Our method is applicable to both discriminative and generative tasks and leads to significant performance improvements in image and text classification, text summarization, multiple-choice QA, and automatic evaluation of generated text. We also extend our method to the "frugal" setting where it is desired to reduce the number of expert model evaluations at test time. Our implementation is publicly available at https://github.com/hwang595/FoE-ICLR2024.

==> YK-macros.tex <==

\def\Avar{\textrm{Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{\textrm{aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{\textrm{avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{\textrm{bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{\textrm{Ber}}
\def\bin{\textrm{bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{\textrm{cat}}
\def\Cov{\textrm{Cov}}
\def\cov{\textrm{cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{\textrm{cl}}
\def\complex{{\bbC}}
\def\cone{\textrm{cone}}
\def\conv{\textrm{conv}}
\def\deq{\overset{d}{=}}
\def\det{\textrm{det}}
\def\diag{\textrm{diag}}
\def\diam{\textrm{diam}}
\def\dist{\textrm{dist}}
\def\dom{\textrm{dom}}
\def\doop{\textrm{do}}
\def\dto{\overset{d}{\to}}
\def\Ex{{\bE}}
\def\Exp{\textrm{Exp}}
\def\exp{\textrm{exp}}
\def\eg{{\it e.g.}}
\def\epi{\textrm{epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\IID{\textrm{IID}}
\def\ind{\textrm{ind}}
\def\intr{\textrm{int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{\textrm{KL}}
\def\ker{\textrm{ker}}
\def\lspan{\textrm{span}}
\def\maximize{\textrm{maximize}}
\def\med{\textrm{med}}
\def\minimize{\textrm{minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{\textrm{Poi}}
\def\Pr{{\bP}}
\def\peq{\overset{p}{=}}
\def\plim{\textrm{plim}}
\def\proj{\textrm{proj}}
\def\prox{\textrm{prox}}
\def\pto{\overset{p}{\to}}
\def\ran{\textrm{ran}}
\def\rank{\textrm{rank}}
\def\reals{{\bR}}
\def\relint{\textrm{relint}}
\def\sign{\textrm{sign}}
\def\st{\textrm{st}}
\def\subjectto{\textrm{subject to}}
\def\supp{\textrm{supp}}
\def\symm{{\bS}}

\def\Tr{\textrm{Tr}}
\def\tr{\textrm{tr}}
\def\tube{\textrm{tube}}
\def\TV{\textrm{TV}}
\def\unif{\textrm{unif}}
\def\Var{\textrm{Var}}
\def\var{\textrm{var}}
\def\vct{\textrm{vec}}
\def\veps{\varepsilon}
\def\vol{\textrm{vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-envs.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{result}[theorem]{Result}


==> backup_folder/experiment_sep28th.tex <==
\vspace{-2mm}
\section{Experiments}
\vspace{-1mm}
We evaluated the efficacy of the FoE method using a wide range of experiments, including image classification, summarization, text generation evaluation, sentiment analysis, and massive multitask language understanding (MMLU) \citep{hendrycks2021measuring}, on various real-world datasets. Additionally, we investigated how to enhance FoE's efficiency, aiming to achieve the desired accuracy while consulting the fewest number of experts, i.e., FrugalFoE. Our results indicate that FoE matches the performance of the "{\it oracle model}" (\ie, always selecting the most suitable expert for a given task) and consistently surpasses individual experts and other popular baseline methods (including FrugalML~\citep{chen2020FrugalML}, ensemble) by a notable margin. Interestingly, FoE inherently tends to be frugal in summarization and sentiment analysis tasks. Specifically, relying on information from just one expert often yields results as effective as consulting all experts. For tasks where FoE is not naturally frugal, our shortest-path algorithm proves effective. For instance, in the CIFAR experiment, FrugalFoE consulted only 37.5\% of the experts to match the accuracy achieved by consulting all of them. 

\vspace{-2mm}
\subsection{Tasks and Experimental Setups}
\vspace{-1mm}
In this section, we briefly discuss the tasks and setups of our experiments. More details about the experimental setup and hyper-parameters used in our experiments can be found in Sections~\ref{sec:appendix-cifar-details}~\ref{sec:appendix-text-gen-eval-details}~\ref{sec:appendix-mmlu-details}~\ref{sec:appendix-sent-analysis-details} of the Appendix. %\my{reference}.
\vspace{-2mm}
\paragraph{CIFAR-100 super-class classification.}
% We evaluate the performance of FoE on an image classification task where the CIFAR-100. 
The CIFAR-100 dataset contains 20 super-classes, each with five sub-classes (100 classes in total)~\cite{krizhevsky2009learning}. We partition CIFAR-100 into 20 sections where each section contains all images from 30 sub-classes. Out of these 30 sub-classes, 20 come exclusively from one sub-class of each super-class (for instance, {\it beaver} from {\it aquatic mammals}, {\it bottles} from {\it food containers}, etc), while the remaining 10 are picked at random from all the other sub-classes. Thus, these sections have overlapping images, meaning they are not mutually exclusive. We train 20 experts, each of them using ResNet-18 on their own data partition conducting super-class classification~\citep{he2016deep}. This partitioning strategy (inspired partly by~\citet{santurkar2021breeds}) ensures that each expert excels in classifying one sub-class within each super-class, however, they have some shared knowledge (more details on final partition can be found in the Appendix). To construct features for training the fusing strategy in FoE (\ie, a classifier to directly predict labels), we use the softmax scores of the last layer for each expert. We use $40k$ images from the CIFAR-100 training set for partitioning and expert training and hold $10k$ images from the training set out as a validation set to train our fusing strategy. Final test accuracy is measured using CIFAR test set.

\vspace{-2mm}
\paragraph{Summarization.} We use fine-tuned Pegasus models on six downstream summarization tasks, 
%\ie, CNN Daily Mail (CNN DM), XSUM, Multi-News, Billsum, Big-Patent, AESLC~\cite{hermann2015teaching,fabbri2019multi, zhang2019email} 
with all the model checkpoints taken from Hugging Face. Here, each fine-tuned model is naturally an expert on corresponding downstream task, \eg, CNN DM. To construct features for fusing strategy training, we take the output embedding of a Pegasus model and average across the context length dimension.
% , taking inspiration from techniques to detect the OOD ~\cite{ren2023outofdistribution}.
We use the combined validation datasets from all six downstream tasks to train the fuser for expert prediction. The true label indicates the source downstream task of the input text sequence/article. For testing, we combined the test sets from all tasks and used ROUGE-2 \citep{lin2003automatic} and BART \citep{yuan2021bartscore} scores to assess the performance.
\vspace{-2mm}
\paragraph{Text generation evaluation.} %Automatic evaluating text generation is fundamental due to the rise of machine language generation but it is still hard to accomplish in many aspects \citep{he2022blind}. In particular,
We investigate the potential of using complementary experts to evaluate machine-generated summaries. For this experiment, we use human-annotated summary datasets namely SummEval \citep{fabbri2021summeval}, Newsroom \citep{grusky2018newsroom}, QAGS-CNN/XSUM \citep{wang2020asking}, and HALL-XSUM \citep{maynez_acl20}. Each dataset has scores for specific dimensions such as coherence and consistency. To train and evaluate experts for each one of the datasets/domains, we: (i) extract some automatic metrics, \eg, BARTScore \citep{yuan2021bartscore}, BERTScore. \my{something is wrong here} Free \citep{shen2022evaluation}, Unieval \citep{zhong2022towards}, from summaries; (ii) randomly select training and test points from each dataset; (iii) for each pair domain/dimension, we train a linear model (expert) that optimally combines precomputed metrics. In total, we have eleven experts; however, experts are only used to evaluate the specific dimension they were trained on. More details on this experiment's setup can be found in Section~\ref{sec:appendix-text-gen-eval-details} of the Appendix.


%yuan2021bartscore Bart
%zhang2019bertscore shen2022evaluation BS
%zhong2022towards UE
%grusky2018newsroom NR
%wang2020asking QAGS
%maynez_acl20 HALXSUM
\vspace{-2mm}
\paragraph{Sentiment analysis.} We use fine-tuned sentence classification models 
 on various sentiment classification tasks as experts in this experiment. The fine-tuned models are from Hugging Face (more details can be found in Section~\ref{sec:appendix-sent-analysis-details} of the Appendix). We have evaluated on Twitter Sentiment Analysis, Twitter Financial Dataset, Poem Sentiment, Data Reviews Sentiment Analysis, 
Auditor Sentiment~\citep{paws2019naacl,sheng2020investigating} from Hugging Face. To train the fusing strategy, we use the input embedding (averaged across the context length dimension) as the feature. Similar to the summarization experiment, the true label indicates the source downstream task of the input text sequence/article. We align the sentiment labels such that all tasks only contain positive and negative sentiments (all other sentiment data are filtered, details can be found in the Appendix). To test we combined the test sets from all tasks.

\vspace{-2mm}
\paragraph{MMLU.} The MMLU test has $57$ tasks including elementary mathematics, US history,  and more~\citep{hendrycks2021measuring}. In this experiment, we selected $15$ open-source LLMs with sizes of $\sim 7$ billion parameters from the Open LLM Leaderboard~\citep{open-llm-leaderboard} (the details are specified in the Appendix). We consider an LLM with the highest accuracy on a category to be an expert for this category.
% to be an expert for a For each category in the test, we select the LLM with the highest accuracy as the category expert.
To construct the feature to learn the fusing strategy, we use the input (without the answer choices) in the MMLU test as the prompt and generate output with maximum sequence length of $16$. We average across the sequence length dimension (prompt and generated tokens) of the last decoder block and use that as the feature for each API. We combine and concatenate all training and validation splits from all categories in the MMLU dataset to train the fusing strategy in FoE. We combine test splits from all categories of MMLU for testing the performance.

\vspace{-2mm}
\subsection{Baseline Methods}
\vspace{-1mm}
For all experiments, we evaluate the performance of individual experts, the "oracle models", and compare them to FoE. We also compare FoE against the vanilla ensemble, uncertainty quantification \my{what is this? lets just call it confidence or max softmax}, and FrugalML~\citep{chen2020FrugalML} as baseline methods when applicable.

\vspace{-2mm}
\subsection{The Performance of Model Fusion with Complementary Expertise}
\vspace{-1mm}
%We first study the performance of FoE over a few practical tasks, including image classification, summarization, sentiment analysis, and multitask language understanding on MMLU.

%\begin{table}[ht]
\begin{wraptable}{r}{0.53\textwidth}
\centering
\vspace{-4mm}
\caption{Image classification task (\ie, CIFAR-100 super-class classification).}
\vspace{-2mm}
\label{tab:accuracy}
{\tiny
\begin{tabular}{l|cc}
\toprule
 \rowcolor{Gray} Method & Final Acc. (\%) & Expert Selection Acc. (\%) \bigstrut\\
\midrule
 FoE & {\bf 82.13} & {\bf 75.27}  \bigstrut\\
\rowcolor{cornsilk} Experts Average & 50.04$_{\pm \text{1.56}}$  & $-$  \bigstrut\\
 Uncertainty-based Fusion & 74.07 & 59.69  \bigstrut\\
\rowcolor{cornsilk} Ensemble & 76.64 & $-$  \bigstrut\\
 Oracle Expert & 87.63 & $-$  \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:cifar-exps}
\vspace{-2mm}
%\end{table}
\end{wraptable}

\vspace{-2mm}
\paragraph{Image classification.} The results of the image classification experiments are shown in Table~\ref{tab:cifar-exps}. In the uncertainty-based fusing baseline, we used the maximum softmax score as an indicator of a model's confidence and then chose the model with the highest confidence for predictions~\citep{guo2017calibration}. We incorporated mix-up, a technique known to enhance the calibration of uncertainty quantification methods, particularly with methods like the max softmax score~\citep{zhang2018mixup}. Additionally, we show the accuracy of an oracle classifier, which operates under the assumption that each test sample is always evaluated using the ideal expert — that is, the expert trained on the data containing the subclass of the the test sample. Our results demonstrate that using FoE markedly improves accuracy over individual experts. FoE also outperforms the uncertainty-based fusion approach and a basic ensemble method, both in prediction accuracy and in expert selection. Notably, FoE's performance comes close to matching the accuracy of the oracle expert.

\vspace{-2mm}
\paragraph{MMLU.} The MMLU experimental results are shown in Table~\ref{tab:mmlu-exps}. Here we report the results of FoE, Oracle experts (always select the highest score among the 15 evaluated LLMs for all MMLU categories), and the average of experts. Due to the space limit, we only show the scores of six sampled MMLU categories, the complete scores can be found in the Appendix. The trained fusing strategy achieves $74.8\%$ expert selection accuracy among 15 experts. Our results demonstrate that FoE leads to effective improvement over individual experts on all MMLU categories and the overall MMLU score (using the 5-shot evaluation following the setting in \citet{eval-harness}) and the performance of FoE is close to oracle expert.
\begin{table}[ht]
\centering
\vspace{-2mm}
\caption{MMLU task experiments, scores of overall accuracy across all 57 test categories, and breakdown accuracy of six selected MMLU categories are reported (breakdown accuracy of the other MMLU categories can be found in the Appendix).}
\vspace{-2mm}
\label{tab:accuracy}
{\tiny
\begin{tabular}{l|cccccc|l}
\toprule
 \rowcolor{Gray} Method & High Scho. EuroHist. & Busi. Ethi. & Coll. Comp. Sci. & Medi. Gene. & Econ. & High Scho. USHist. & Overall. \bigstrut\\
\midrule
FoE & 68.29 & 45.45 & 40.40 & 68.69 & 36.28 & 67.45 & 49.85 \bigstrut\\
\rowcolor{cornsilk} Oracle Expert & 68.90 & 51.52 & 45.45 & 69.70 & 40.71 & 70.94 & 51.56 \bigstrut\\
Avg. Experts & 54.11$_{\pm \text{15.61}}$ & 42.96$_{\pm \text{10.30}}$ & 36.77$_{\pm \text{6.92}}$ & 52.05$_{\pm \text{11.20}}$ & 30.80$_{\pm \text{4.90}}$ & 54.98$_{\pm \text{16.51}}$ & 41.34$_{\pm \text{7.22}}$ \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:mmlu-exps}
\vspace{-3mm}
\end{table}

\begin{table}[ht]
\centering
\caption{Summarization task experiments, ROUGE-2 score (higher is better) as the evaluation metric.}
\vspace{-2mm}
\label{tab:accuracy}
{\tiny
\begin{tabular}{l|llllll|l}
\toprule
 \rowcolor{Gray} Method & CNN DM & XSUM & Multi-News & BillSum & Big-Patent & AESLC & Avg. \bigstrut\\
\midrule
 FoE & 20.2225 & 23.8662 & 18.3499 & 36.9398 & 27.0756 & 20.6736 & {\bf 23.7171} \bigstrut\\
\rowcolor{cornsilk} CNN DM Expert & \underline{20.2472} & 3.5595 & 8.2049 & 14.0173 & 12.7726 & 2.4269 & 11.3757 \bigstrut\\
 XSUM Expert & 7.4224 & \underline{23.8904} & 4.0622 & 8.0220 & 11.0968 & 2.9332 & 11.9509 \bigstrut\\
\rowcolor{cornsilk} Multi-News Expert & 10.3799 & 4.8769 & \underline{18.5120} & 7.2528 & 7.0045 & 0.4224 & 8.5559\bigstrut\\
 BillSum Expert & 8.7146 & 3.2458 & 4.6663 & \underline{38.5739} & 6.2896 & 1.9565 & 8.1622 \bigstrut\\
\rowcolor{cornsilk} Big-Patent Expert & 7.2759 & 3.4595 & 4.1817 & 10.4013 & \underline{27.0760} & 0.9100 & 10.2426 \bigstrut\\
AESLC Expert & 5.9838 & 3.6185 & 1.6123 & 4.1015 & 3.0258 & \underline{20.6842} & 4.6352 \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:summ-exps}
\vspace{-2mm}
\end{table}

\vspace{-2mm}
\paragraph{Summarization.} Our summarization experiments are summarized in Table~\ref{tab:summ-exps} where decomposed scores on each downstream task for all experts and FoE are shown. Our trained fusing strategy achieved $99.1\%$ on predicting six experts. One can see that FoE almost reaches the best ROUGE-2 score on each downstream task, \ie, FoE almost reaches the performance of the oracle expert.


\vspace{-0mm}
\begin{wraptable}{r}{0.57\textwidth}
\centering
\vspace{-0mm}
\caption{Sentiment analysis task experiments, where TFN stands for Twitter Financial News.}
\vspace{-2mm}
\label{tab:accuracy}
{\tiny
\begin{tabular}{l|llll|l}
\toprule
 \rowcolor{Gray} Method & TFN & Poem & Auditor & Reviews Sent. & Avg. \bigstrut\\
\midrule
 Model Fuser & 87.54\% & 85.71\% & 81.71\% & 95.20\% & {\bf 91.88}\% \bigstrut\\
\rowcolor{cornsilk} TFN Model & \underline{87.54}\% & 0.0\% & 58.54\% & 0.40\%& 26.85\% \bigstrut\\
Poem Model & 6.69\% & \underline{85.71}\% & 15.24\% & 59.76\% & 46.95\%  \bigstrut\\
\rowcolor{cornsilk} Auditor Model & 51.98\% & 45.71\% & 
 \underline{81.71}\% & 49.65\% & 53.50\%  \bigstrut\\
Reviews Sent. Model & 71.12\% & 62.86\% & 32.93\% & \underline{95.20}\% & 79.44\% \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:sent-analysis-exps}
\vspace{-4mm}
%\end{table}
\end{wraptable}
\paragraph{Sentiment analysis.} Our sentiment analysis experiments are summarized in Table~\ref{tab:sent-analysis-exps} where decomposed scores on each downstream task for all experts and FoE are shown. Our trained fusing strategy achieved $99.1\%$ on predicting four experts. One can see that FoE almost reaches the best sentiment classification accuracy on each downstream task, \ie, FoE almost reaches the performance of the oracle expert.
%\begin{table}[ht]

\vspace{-2mm}
%\begin{table}[ht]
\begin{wraptable}{r}{0.7\textwidth}
\vspace{-4mm}
\centering
\caption{Summary evaluation, Pearson correlation of human labels and automated metrics}
\vspace{-2mm}
{\tiny
\begin{tabular}{l|cccccc}
\toprule
\rowcolor{Gray}  Method& SummEval & NEWSROOM & H-XSUM & Q-CNN & Q-XSUM & Avg. \bigstrut\\
\midrule
Model Fuser & 0.613 & 0.652 & 0.237 & 0.738 & 0.343 & {\bf 0.517} \bigstrut\\
\rowcolor{cornsilk}SummEval Expert & \underline{0.655} & 0.51 & 0.209 & 0.716 & \underline{0.357} & 0.489 \bigstrut\\
NEWSROOM  Expert & 0.293 & \underline{0.685} & 0.167 & 0.673 & 0.112 & 0.386 \bigstrut\\
\rowcolor{cornsilk}H-XSUM  Expert & 0.548 & 0.592 & 0.241 & \underline{0.747} & 0.348 & 0.495 \bigstrut\\
Q-CNN  Expert & 0.502 & 0.612 & 0.237 & \underline{0.747} & 0.337 & 0.487 \bigstrut\\
\rowcolor{cornsilk}Q-XSUM  Expert & 0.499 & 0.586 & \underline{0.243} & 0.729 & 0.323 & 0.476 \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:summ-eval}
\vspace{-4mm}
%\end{table}
\end{wraptable}
\paragraph{Text generation evaluation.} We compare the performances of FoE and individual experts in evaluating the consistency\footnote{Consistency/factuality measures if the facts presented in the summary are consistent with those presented in the source text. In the Newsroom dataset, this dimension is termed as ``relevance". Please check Table \ref{tab:summ-eval-append} in the Appendix for the full table.} (or factuality) of machine-generated summaries. Because each dataset has a different format for the human annotations, experts' outputs are not comparable, and we cannot compute the aggregate correlation of predictions and human labels for a given task (pair dataset/dimension) when evaluating FoE. Instead, we estimate the expected conditional correlation between predictions and human labels in the following way: using the outputs from the eleven experts and for each domain, we classify each text in the test set according to their dataset membership, and according to the empirical distribution of classes induced by the classifier, we compute a weighted average of the correlations achieved by experts in that specific task \my{stuff about correlation computation is a minor detail and can go to appendix}. In Table \ref{tab:summ-eval}, we can see that, for individual tasks, Model Fuser does not lead to the highest correlations; however, with aggregated correlations in the last column, our approach delivers the overall best results.

\vspace{-2mm}
\subsection{FrugalFoE Experiments}
\vspace{-1mm}
To achieve FrugalFoE, we aim at querying as small a number of experts as possible. In this section, we measure the performance of our shortest path algorithm using two fusing strategy models, \ie, neural networks and $k$-nearest neighbors. For kNN experiments, we used $\kappa=9$. For both kNN and NN experiments, we vary the selection of $M$ and $\lambda$ to control the number of experts we end up with querying. For the NN experiments, since we cannot traverse the entire $2^K-1$ search space in the shortest path graph we tried to explore all possibilities on querying up to 5 experts.

\vspace{-2mm}
\paragraph{Shortest path FrugalFoE.} The FrugalMoE results are shown in Figure~\ref{fig:frugalmoe} where one can observe that (especially for the kNN experiment) FrugalFoE can use $37.5\%$ of the experts to reach the accuracy of using the entire 20 experts on the CIFAR task. When querying the same number of experts (FrugalML constraints itself by only allowing querying at most two experts), FrugalFoE achieves better accuracy than FrugalML.
\begin{figure*}[ht]
    \vspace{-3mm}
    \centering
    \subfigure[kNN as classifiers]{\includegraphics[width=0.32\textwidth]{figures/frugal_fuser_knn.pdf}}
    \subfigure[NN as classifiers]{\includegraphics[width=0.32\textwidth]{figures/frugal_fuser_nn_bs.pdf}}
    \vspace{-3mm}
    \caption{FrugalFoE results on the CIFAR-100 super-class classification task.}
    \label{fig:frugalmoe}
    \vspace{-3mm}
\end{figure*}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/frugal_fuser_knn.pdf}
%     \caption{Frugal CIFAR-100 fuser.}
%     \label{fig:frugal-fuser-cifar100}
% \end{figure}

\vspace{-2mm}
\paragraph{Natural FrugalFoE.} Surprisingly, in the summarization and sentiment analysis experiments the FoEs are naturally frugal. More specifically, even solely using one expert's feature to train the fusing strategy can make the model fuser work well. Here the results are shown in Table~\ref{tab:model-fuser-summarization-single-api} and Table~\ref{tab:frugal-sent-analysis-exps} where one can see even using a single expert's output as a feature to train the fusing strategy, the end FoEs can still perform well (as well as using all experts' feature and close to the orcale classifier).
\begin{table}[ht]
\vspace{-2mm}
\centering
\caption{Summarization task experiments, ROUGE-2 score as evaluation metric. The feature used in this experiment is solely from each individual API.}
\vspace{-2mm}
\label{tab:model-fuser-summarization-single-api}
{\tiny
\begin{tabular}{l|llllll|l}
\toprule
 \rowcolor{Gray} Method & CNN DM & XSUM & Multi-News & BillSum & Big-Patent & AESLC & Avg. \bigstrut\\
\midrule
 Model Fuser & 20.2225 & 23.8662 & 18.3499 & 36.9398 & 27.0756 & 20.6736 & 23.7171 \bigstrut\\
\rowcolor{cornsilk} CNN DM feature only & 20.1599 & 23.7911 & 18.1450 & 37.8557 & 27.0765 & 20.5473 & 23.7180 \bigstrut\\
 XSUM feature only & 20.1402 & 23.8484 & 18.0158 & 36.3483 & 27.0709 & 20.5520 & 23.5963 \bigstrut\\
\rowcolor{cornsilk} Multi-News feature only & 19.8900 & 23.3156 & 17.7478 & 18.1870 & 27.0660 & 20.3217 & 21.9752 \bigstrut\\
BillSum feature only & 19.5018 & 23.0579 & 17.5037 & 31.6007 & 27.0413 & 20.3720 & 22.7815 \bigstrut\\
\rowcolor{cornsilk} Big-Patent feature only & 19.3697 & 22.6215 & 17.0606 & 37.0621 & 27.0731 & 20.1715 & 22.9850 \bigstrut\\
AESLC feature only & 20.0286 & 23.6388 & 17.8641 & 37.8359 & 27.0661 & 20.3707 & 23.5954 \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:summ-exps}
\vspace{-3mm}
\end{table}

\begin{table}[ht]
\centering
\vspace{-2mm}
\caption{Sentiment analysis task experiments, where TFN stands for Twitter Financial News.}
\vspace{-2mm}
\label{tab:accuracy}
{\tiny
\begin{tabular}{l|llll|l}
\toprule
 \rowcolor{Gray} Method & TFN & Poem & Auditor & Reviews Sent. & Avg. \bigstrut\\
\midrule
 Model Fuser & 87.54\% & 85.71\% & 81.71\% & 95.20\% & {\bf 91.88}\% \bigstrut\\
\rowcolor{cornsilk} TFN Feature Only & 86.93\% & 85.71\% & 82.32\% & 95.20\% & 91.81\% \bigstrut\\
Poem Feature Only & 87.23\% & 82.86\% & 81.10\% & 95.20\% & 91.75\%  \bigstrut\\
\rowcolor{cornsilk} Auditor Feature Only & 86.32\% & 82.86\% & 
 82.32\% & 95.20\% & 91.62\%  \bigstrut\\
Reviews Sent. Feature Only & 87.23\% & 85.71\% & 81.10\% & 95.20\% & 91.88\% \bigstrut\\
\bottomrule
\end{tabular}}
\label{tab:frugal-sent-analysis-exps}
\vspace{-3mm}
\end{table}
